Belonging Beyond Code: Queer Software Engineering and Humanities Student Experiences

Queer students often encounter discrimination and a lack of belonging in their academic environments. This may be especially true in heteronormative male-dominated fields like software engineering, which already faces a diversity crisis. In contrast, disciplines like humanities have a higher proportion of queer students, suggesting a more diverse academic culture. While prior research has explored queer students' challenges in STEM fields, limited attention has been given to how experiences differ between the sociotechnical, yet highly heteronormative, field of software engineering and the socioculturally inclusive humanities. This study addresses that gap by comparing 165 queer software engineering and 119 queer humanities students experiences. Our findings reveal that queer students in software engineering are less likely to be open about their sexuality, report a significantly lower sense of belonging, and encounter more academic challenges compared to their peers in the humanities. Despite these challenges, queer software engineering students show greater determination to continue their studies. These insights suggest that software engineering could enhance inclusivity by adopting practices commonly seen in the humanities, such as integrating inclusive policies in classrooms, to create a more welcoming environment where queer students can thrive.

==> content/tables/questionnaire2.tex <==
\begin{table}[tb]
\centering
\caption{Questionnaire for students (\textit{RQ3, RQ4})}
\label{tab:questionnairestudentsRQ3RQ4}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lp{6.5cm}l}
\toprule
Var. & Question & Source\\
\midrule
\belowrulesepcolor{gray!25}
\rowcolor{gray!25}\multicolumn{3}{l}{Sense of Belonging (RQ3)} \\
\aboverulesepcolor{gray!25}
SB01\_01	& How much do you interact socially with other students in your studies? & \cite{mooney2021investigating} \\
SB01\_02	& How well do people in your current field of study understand you as a person? & \cite{senseofbelongingScale2020} \\
\midrule
SB01\_03	& How connected do you feel to the university staff in your current field of study? & \cite{senseofbelongingScale2020} \\
SB01\_04	& How welcoming have you found your current field of study to be? & \cite{senseofbelongingScale2020} \\
\midrule
SB01\_05	& How much respect do other students in your current field of study show toward you? & \cite{senseofbelongingScale2020} \\
SB01\_06	& How much respect do members of staff in your current field of study show toward you? & \cite{senseofbelongingScale2020} \\
SB01\_07	& How much do you matter to others in your current field of study? & \cite{senseofbelongingScale2020} \\
\midrule
SB01\_08 & How happy are you with your choice to be a student in your current field of study? & \cite{senseofbelongingScale2020} \\
SB01\_09 & How enriching is your experience in your current field of study? & \cite{senseofbelongingScale2020} \\
SB01\_10 & How 'at home' do you feel in your current field of study? & \cite{senseofbelongingScale2020} \\
\midrule
SB01\_11 & Overall, how much do you feel like you belong in your current field of study? & \cite{senseofbelongingScale2020} \\ 

\midrule
\belowrulesepcolor{gray!25}
\rowcolor{gray!25}\multicolumn{3}{l}{Drop Out Rate (RQ 4)} \\
\aboverulesepcolor{gray!25}
 DP01 &	During your academic career, have you ever seriously considered leaving your graduate program? & \cite{stout2016lesbian} \\
 DP02 &	Please briefly explain your answer to the prior question.  & \cite{stout2016lesbian} \\
 
%CS01	& Do you have coping strategies, if you struggle in your studies based on your sexuality? & [new] \\
%CS02 & Please briefly explain your answer to the prior question. & [new] \\
%CS03 & Do these coping strategies affect your wellbeing? & [new] \\
%CS04 & Please briefly explain your answer to the prior question. & [new] \\

%\midrule
%\belowrulesepcolor{gray!25}
%\rowcolor{gray!25}\multicolumn{3}{l}{Enhance queer students experience (RQ4)} \\
%\aboverulesepcolor{gray!25}
%CC03	& Have you personally experienced any inclusive (e.g., welcomed, acknowledged), encouraging, pleasant and/or friendly conduct (supportive behavior) that has positively impacted your ability to learn or your wellbeing in your current field of study because of your sexual orientation, or sexual identity? & [new] \\
%CC04	& If you answered the previous question with yes, can you please describe these scenarios? \isa{TBA analysis}& [new] \\
%CS05 & Do you feel self-empowered by doing your major despite hardships based on your sexuality? & [new] \\
%CS06 & Please briefly explain your answer to the prior question. & [new] \\



\bottomrule
\end{tabular}%
}
\end{table}

==> content/tables/rq1_sb.tex <==
\begin{table*}[tb]
    \centering
    \small
    \caption{Sense of belonging in queer students (p-value, A12)}
\begin{tabular}{llllll}
\toprule
 & total: cs vs ha & hetero: cs vs ha & queer: cs vs ha & queer cs vs hetero cs & queer ha vs hetero ha \\
\midrule
SB01\_01 & 0.26, 0.46 & 0.98, 0.5 & 0.16, 0.45 & 0.28, 0.44 & 0.93, 0.51 \\
SB01\_02 & 0.21, 0.46 & 0.93, 0.49 & 0.12, 0.44 & 0.24, 0.44 & 0.79, 0.47 \\
SB01\_03 & 0.64, 0.48 & 0.94, 0.49 & 0.39, 0.47 & 0.11, 0.42 & 0.55, 0.44 \\
SB01\_04 & \textbf{0.02}, 0.42 & 0.65, 0.45 & \textbf{0.01}, 0.4 & 0.08, 0.41 & 0.75, 0.47 \\
SB01\_05 & 0.15, 0.45 & 0.76, 0.47 & \textbf{0.05}, 0.43 & \textbf{0.04}, 0.4 & 0.47, 0.43 \\
SB01\_06 & 1.0, 0.5 & 0.48, 0.43 & 0.73, 0.49 & 0.06, 0.41 & 0.12, 0.35 \\
SB01\_07 & 0.42, 0.47 & 0.98, 0.5 & 0.37, 0.47 & 0.67, 0.48 & 0.98, 0.5 \\
SB01\_08 & 0.14, 0.55 & 0.23, 0.62 & 0.41, 0.53 & 0.16, 0.43 & 0.87, 0.52 \\
SB01\_09 & 0.15, 0.45 & 0.57, 0.44 & 0.11, 0.44 & 0.27, 0.44 & 0.61, 0.45 \\
SB01\_10 & 0.19, 0.46 & 0.54, 0.56 & 0.09, 0.44 & 0.24, 0.44 & 0.53, 0.56 \\
SB01\_11 & 0.43, 0.47 & 0.57, 0.56 & 0.15, 0.45 & \textbf{0.02}, 0.39 & 0.92, 0.51 \\
\bottomrule
\label{tab:rq1_sb}
\end{tabular}
\end{table*}
